Constructing LDPC Codes by 2-Lifts

We propose a new low-density parity-check code construction scheme based on 2-lifts. The proposed codes have an advantage of admitting efficient hardware implementations. With the motivation of designing codes with low error floors, we present an analysis of the low-weight stopping set distributions of the proposed codes. Based on this analysis, we propose design criteria for designing codes with low error floors. Numerical results show that the resulting codes have low error probabilities over binary erasure channels.

==> conclusion.tex <==
\section{Conclusion}

\label{sec_conclusion}

This paper proposes a new construction schemes for LDPC codes based
on random $2$-lift. We present an analysis for low-weight stopping
set distributions. Based on this analysis, we propose design
criteria for the resulting codes to have low error floors. Numerical
results show that the proposed codes outperform the previously
constructed codes in terms of error probability performance.


==> intro.tex <==
\section{Introduction}



Low-Density Parity-Check (LDPC) codes receive much attention
recently. The advantages of the codes include capacity-approaching
performance for many important channels, and highly efficient
parallel decoding algorithms.

The {\it protograph based} LDPC codes are a class of LDPC codes
constructed by random $N$-lifts of small Tanner graphs
\cite{thorpe}. A major advantage of protograph based LDPC codes is
that decoding can be efficiently implemented by a semi-parallel
hardware structure \cite{lee04}. Several protograph based LDPC code
ensembles with low error probabilities are also previously reported,
for example, \cite{divsalar05a}, \cite{divsalar05b},
\cite{divsalar05c}.


In this paper, we propose a new LDPC code construction scheme based
on a series of random $2$-lifts. The proposed code ensembles are
subsets of protograph based code ensembles by $2^n$-lifts, where $n$
is a positive integer. As with the protograph based codes, decoding
of the proposed codes can be efficiently implemented by the same
semi-parallel hardware structure. In addition, the description
complexity of the proposed codes is lower than that for conventional
protograph based codes.


It is well known that LDPC codes may exhibit error floors. The error
floors are caused by small subgraphs with certain structures in the
corresponding Tanner graphs \cite{richardson03}, \cite{mackay03},
\cite{di02}, \cite{forney01}. One of the above subgraph structures
is the so called {\it stopping set}.


In order to understand and predict the performance of LDPC codes,
previous research has proposed several approaches on approximately
calculating stopping set distributions and codeword distributions
\cite{burshtein}, \cite{fogal}. These previous approaches determine
the exact values of limiting exponents by large deviation
principles; in here, exponents are defined as the logarithms of the
numbers of codewords or stopping sets with certain relative
distances, normalized by the blocklengths.

For properly designed LDPC codes, the limiting exponents with
respect to blocklengths are typically negative for low relative
distances and zero for vanishing relative distances. In other words,
low-weight stopping sets are typically stopping sets with vanishing
relative distances; the number of these low-weight stopping sets
scales sub-exponentially with respect to blocklength. These
potentially existing low-weight stopping sets result in high error
floors. It is desirable that these low-weight stopping sets are
avoided.




\comment{ However, for LDPC codes with bounded degrees, the
exponents of stopping set distributions and codeword distributions
with vanishing relative distances are typically zero. In other
words, the numbers of stopping sets with low weights grow
sub-exponentially with respect to codeword lengths. Knowing
exponents along is not sufficient to determine the error probability
performance because the sub-exponentially scaling numbers of
low-weight stopping sets could have large impacts on the overall
error probability performance. Therefore, it is crucial to know the
order of the sub-exponential scaling law, with which the numbers of
low-weight stopping sets grow. However, to our best knowledge, there
is no existing method to address this problem.}





In this paper, we present an analysis of low-weight stopping set
distributions of the proposed codes in terms of graph expansion
properties. We show that low-weight stopping sets can be largely
avoided if the protograph satisfies certain graph expansion
properties. Based on this analysis, we propose design criteria for
the proposed $2$-lift based codes to have low error floors. Several
numerical examples of code design using the design criteria are
presented. The numerical results confirm our theoretical analysis.






 The rest of this paper is organized as follows. In Section~\ref{sec_pre},
 we introduce notations and backgrounds. The proposed code construction scheme
 is shown in Section~\ref{sec_lift}. In Section \ref{sec_weight}, we present the
analysis on low-weight stopping set distributions. Remarks and
discussions are presented in Section \ref{sec_discussion}. Based on
the above discussions, a set of design criteria is presented. The
proof is shown in Section \ref{sec_proof}. We present numerical
results in Section \ref{sec_numerical}. Conclusions are given in
Section \ref{sec_conclusion}.
































%

